Modeling the Influence of Visual Density on Cluster Perception in Scatterplots Using Topology

Scatterplots are used for a variety of visual analytics tasks, including cluster identification, and the visual encodings used on a scatterplot play a deciding role on the level of visual separation of clusters. For visualization designers, optimizing the visual encodings is crucial to maximizing the clarity of data. This requires accurately modeling human perception of cluster separation, which remains challenging. We present a multi-stage user study focusing on four factors---distribution size of clusters, number of points, size of points, and opacity of points---that influence cluster identification in scatterplots. From these parameters, we have constructed two models, a distance-based model, and a density-based model, using the merge tree data structure from Topological Data Analysis. Our analysis demonstrates that these factors play an important role in the number of clusters perceived, and it verifies that the distance-based and density-based models can reasonably estimate the number of clusters a user observes. Finally, we demonstrate how these models can be used to optimize visual encodings on real-world data.

==> sec-experiment-results-density-differ-table.tex <==

\begin{table*}[!ht]
        \centering
        \caption{Density-based model Repeated-Measures ANOVA results on the effect of visual factors for user response accuracy (i.e., \textit{differential}), $\Dspace_{de}^*$.}
        \label{table:tab-density-threshold}
        %       \vspace{.25in}
        \resizebox{1.0\linewidth}{!}{%
        \begin{tabular}{@{\extracolsep{6pt}}c@{}c||@{}c@{}c@{}c@{}c@{ }|@{ }c@{ }c@{ }c@{ }c@{ }|@{ }c@{ }c@{ }c@{ }c@{ }|@{ }c@{ }c@{ }c@{ }c@{ }|@{ }c}
        & & \multicolumn{4}{c}{\underline{Distribution Size (S)}}& 
                     \multicolumn{4}{c}{\underline{Number of Points (N)}} & 
                     \multicolumn{4}{c}{\underline{Point Size (P)}} & 
                     \multicolumn{4}{c}{\underline{Interaction (N*P)}} \\
                 Model & Grid & Df & F-val & P-val & $\eta_{}^{2}$  &  Df & F-val & P-val & $\eta_{}^{2}$ & Df & F-val & P-val & $\eta_{}^{2}$ & Df & F-val & P-val & $\eta_{}^{2}$ & $\sigma$ \\
                %  \CLINE{2-4}\CLINE{5-7}\CLINE{8-10}
                 \hline \hline
                                      & $10_{px}\times10_{px}$ & 4 &  061.45 & $\leq$ 0.001 & 0.090  & 2 & 122.60 & $\leq$ 0.001 & 0.090  & 3 & 086.28 & $\leq$ 0.001 & 0.099 & 6 &  11.28 & $\leq$ 0.001   & 0.028 & 1.640\\
                \rowcolor{lightergray}
                $\Dspace_{de}^{N}$  & $20_{px}\times20_{px}$ & 4 &  014.99 & $\leq$ 0.001 & 0.020  & 2 &  058.80 & $\leq$ 0.001 & 0.045 & 3 & 301.80 & $\leq$ 0.001 & 0.280  & 6 &  10.20  & $\leq$ 0.001   & 0.025 & 1.760\\
                                      & $40_{px}\times40_{px}$ & 4 & 129.22 & $\leq$ 0.001 & 0.180  & 2 & 216.00 & $\leq$ 0.001 & 0.150  & 3 & 613.20 & $\leq$ 0.001 & 0.430  & 6 &  56.90  & $\leq$ 0.001   & 0.120  & 2.440\\
                \hline
                                      & $10_{px}\times10_{px}$ & 4 &  088.58 & $\leq$ 0.001 & 0.130  & 2 &  096.50 & $\leq$ 0.001 & 0.075 & 3 &   006.00 & $\leq$ 0.001 & 0.086 & 6 &   1.62 & 0.103 & 0.004 & 1.680\\
                \rowcolor{lightergray}
                 $\Dspace_{de}^{P}$   & $20_{px}\times20_{px}$ & 4 &   004.98 & $\leq$ 0.001 & 0.008 & 2 & 143.80 & $\leq$ 0.001 & 0.100  & 3 &  074.30 & $\leq$ 0.001 & 0.080  & 6 &  11.40  & $\leq$ 0.001   & 0.028 & 1.520\\
                                      & $40_{px}\times40_{px}$ & 4 &  094.45 & $\leq$ 0.001 & 0.130  & 2 & 439.70 & $\leq$ 0.001 & 0.270  & 3 & 135.40 & $\leq$ 0.001 & 0.140  & 6 & 010.80  & $\leq$ 0.001   & 0.250  & 2.070\\
                \hline
                                      & $10_{px}\times10_{px}$ & 4 &  057.95 & $\leq$ 0.001 & 0.090  & 2 & 383.90 & $\leq$ 0.001 & 0.240  & 3 & 246.30 & $\leq$ 0.001 & 0.240  & 6 & 130.30  & $\leq$ 0.001  & 0.250  & 1.710\\
                \rowcolor{lightergray}
                 $\Dspace_{de}^{N*P}$ & $20_{px}\times20_{px}$ & 4 &   007.56 & $\leq$ 0.001 & 0.012 & 2 &  047.10 & $\leq$ 0.001 & 0.038 & 3 &  061.20 & $\leq$ 0.001 & 0.070  & 6 &  11.40  & $\leq$ 0.001   & 0.028 & 1.470\\
                                      & $40_{px}\times40_{px}$ & 4 &  062.81 & $\leq$ 0.001 & 0.096 & 2 & 273.30 & $\leq$ 0.001 & 0.180  & 3 & 195.50 & $\leq$ 0.001 & 0.190  & 6 &  19.10  & $\leq$ 0.001   & 0.046 & 1.910\\
                \hline
        \end{tabular}
        }
    
    \vspace{-8pt}
    \begin{flushleft}{\footnotesize 
        \colorbox{lightergray}{The $[20_{px}\times20_{px}]$ grid is highlighted to indicate it is the primary focus of our analysis.} 
    } 
    \end{flushleft}        
    \vspace{-8pt}
    
\end{table*}






==> sec-experiment-results-density.tex <==




   
\input{sec-experiment-results-density-differ-table.tex} 
    

\subsubsection{Density-based Model}
\label{sec.eval.density}


    For the density-based model, we calculate 3 variations of the threshold and differential that use the factors that most directly influence visual density. Those are the {number} of data points ($T_{de}^N$/$\Dspace_{de}^N$), the {size} of data points ($T_{de}^P$/$\Dspace_{de}^P$), and their interaction ($T_{de}^{N*P}$/$\Dspace_{de}^{N*P}$).
    For each, we performed 3-factor RM ANOVA testing on the individual factors the distribution size ($S$), the number of points ($N$), and the point size ($P$), as well as interaction effects (see \autoref{table:tab-density-threshold}). 

    
    \begin{figure}[!b]
        \centering
        
        \begin{minipage}[t]{0.05\linewidth}
            \rotatebox{90}{
    		    \begin{minipage}{2.5cm}
    		    \centering
    		    \footnotesize Normalized Persistence Threshold
    		    \end{minipage}
    		}
    	\end{minipage}
    	\hspace{2pt}
    	\begin{minipage}[t]{0.8\linewidth}	
    	    \centering
            \includegraphics[width=\linewidth]{fig/VD_plot.pdf}
    	\end{minipage}
    	
        \caption{Normalized persistence threshold for the density-based model for the data from \autoref{fig:example_stimuli} shows stability at histogram bins size $[20_{px}\times 20_{px}]$ and larger.}
        \label{fig:VD-plot}
    \end{figure}
   
   
    \para{Histogram Resolution} The density-based model uses the \textit{visual density} of a given scatterplot to model cluster perception. To calculate visual density, a 2D histogram is calculated on the image with bins of uniform width and height, $[B_{px}\times B_{px}]$.    The choice of bin size for the density histogram is potentially influential in our analysis, as bins that are too small may cause instability, and bins that are too large may miss clusters. To determine the appropriate bin size, we performed an analysis on the data from \autoref{fig:example_stimuli}. A set of stimuli images are generated with fixed values for factors ($C=6$, $N=2500$, and $P=7_{px}$) and different values for $S=\{25_{px}, 40_{px}, 55_{px}, 70_{px}, 85_{px}\}$. We plotted the normalized density threshold (i.e., density threshold divided by area of a bin, i.e., $T_{de}/B^2$) generated by $U=6$ clusters for 5 different bin sizes (see \autoref{fig:VD-plot}). The results showed instability in the density threshold for smaller values and a stable result starting at $[20\times20]$. For this reason, 3 resolutions of histogram cell sizes are reported: $[10_{px}\times10_{px}]$, $[20_{px}\times20_{px}]$, and $[40_{px}\times40_{px}]$, but our main discussion focuses on $[20_{px}\times20_{px}]$.
   


       
    \para{Number of Points Model ($T_{de}^{N}$/$\Dspace_{de}^{N}$)} 
    RM ANOVA results demonstrate significant and consistent main effects of $S$, $N$, $P$, and interaction effect of $N*P$, which can be seen in \autoref{table:tab-density-threshold}. Point size has a large effect on $\Dspace_{de}$, confirming our hypotheses and previous work (e.g., \cite{sadahiro1997cluster}) of density's influence on cluster perception. The number of points showed a small-medium effect size on $\Dspace_{de}$, also align with our hypotheses. The accuracy of the number of points model was the worst of the 3 density models, though still significantly better than no model (see \autoref{fig:histogram-density}). The accuracy of the model, plotted by the number of points in \autoref{fig:de_ci:a}, shows lower accuracy as the number of points increases.
   
   

     \para{Point Size Model ($T_{de}^{P}$/$\Dspace_{de}^{P}$)} 
     In this model, the number of points showed a medium-large effect size, while point size demonstrated a medium effect size for the differential. On the other hand, interaction of $N*P$ results small values of $\eta^2$ (see \autoref{table:tab-density-threshold}). The overall accuracy of this model was better than the number of points model (see \autoref{fig:histogram-density}). \autoref{fig:de_ci:b} shows the accuracy per point size. The model was largely accurate, except for the smallest size, $P=1_{px}$.
     


     \para{Interaction Model ($T_{de}^{N*P}$/$\Dspace_{de}^{N*P}$)} 
      Similar to the previous 2 models, significant effects were observed for all factors. However, only point size demonstrated medium effect size (see \autoref{table:tab-density-threshold}). \uline{This model showed the best overall accuracy of any model tested} (see \autoref{fig:histogram-density}). This makes logical sense, as the density is the combination of the number of points and their size. \autoref{fig:de_ci:c} shows the accuracy per number of points and per point size. For both cases, the accuracy was improved. However, $P=1_{px}$ was still the worst performing category.
           
      
      Our analysis showed the number of points, point size, and their interaction all had significant effects and improved accuracy over no model.
      \textbf{Therefore, we consider \ref{Hyp:H5} confirmed}. Furthermore, we identified some large effects with point size for the density-based model, and \textbf{this indirect relationship confirms \ref{Hyp:H3}}.

       

   
\begin{figure}[!t]
    \centering
     \subfigure[$\Dspace_{de}^{N}$ for the number of points\label{fig:de_ci:a}]{\includegraphics[height=1.725cm]{fig/ci_plots/CIPlot_new_de_n.pdf}}
     \hfill
    \subfigure[$\Dspace_{de}^{P}$ for the size of points\label{fig:de_ci:b}]{\hspace{2pt}\includegraphics[trim=0pt 0 0 0, clip, height=1.725cm]{fig/ci_plots/CIPlot_new_de_p.pdf}\hspace{2pt}}
    \hfill
    \subfigure[$\Dspace_{de}^{N*P}$ for the number (left) and size (right) of points.\label{fig:de_ci:c}]{\includegraphics[trim=0pt 0 0 0, clip, height=1.725cm]{fig/ci_plots/CIPlot_new_de_np_n.pdf}
    \hspace{3pt}
    \includegraphics[trim=0pt 0 0 0, clip, height=1.725cm]{fig/ci_plots/CIPlot_new_de_np_p.pdf}}
    \caption{Density-based model mean and $95\%$ confidence intervals of user response differential, $\Dspace_{de}^*$, on factors with density histogram $[20_{px}\times20_{px}]$.}
    \label{fig:de_ci}
\end{figure}
   
       
    
    
\subsubsection{Post-Test Questionnaire}
To further support our hypotheses, we asked the participants to state the criteria that influenced their counting of clusters in a free-response format at the end of the experiment. Their responses largely mirrored our findings---10\% cited the size of symbol; 25\% responses cited something amounting to distribution size; 25\% cited distance between clusters; and 65\% of responses included density as a factor\footnote{Some subjects listed multiple criteria.}. 
    
    
    
    
    
  

==> sec-experiment-results-distance.tex <==



\renewcommand{\arraystretch}{1.1}
\begin{table}[!t]
    \centering
    \caption{Distance-based model Repeated-Measures ANOVA results on the effect of visual factors on the \textit{differential}, $\Dspace_{di}^S$.}
    \label{tbl:factors_distance}
    \resizebox{1.0\linewidth}{!}{%
    \begin{tabular}{l || cc | cc | cc}
        Factors & Df & F-value & P-value & $\eta_{}^{2}$ & $\sigma$  \\
        \hline
        \hline
        
         \quad Distribution size (S) & 4 & 552.9 & $\leq$ 0.001 & 0.4900 & 1.91 \\ % \\
         \quad Number of points (N) & \textcolor{green}{1.98} &  \textcolor{green}{051.39} &  \textcolor{green}{$\leq$ 0.001} & 0.0420 & 2.61 \\    % \\
         \quad Size of points (P) & 3 & 000.41 & 0.746 & 0.0005 & 2.64\\       % \\
         \quad S*N & 8 & 002.72 & 0.006 & 0.0100 & - \\       % \\
         \quad S*P & 12 & 000.13 & 1.000 & 0.0006 & -\\       % \\
         \quad N*P & 6 & 000.08 & 0.998 & 0.0002 & -\\       % \\
         \quad S*P*N & 24 & 000.21 & 1.000 & 0.0020 & -\\       % \\
         \hline
    \end{tabular}} 

    \vspace{-8pt}
    \begin{flushleft}{\footnotesize 
    %*: $p<0.05$; **: $p< 0.01$; 
    -: not calculated; \color{green}{Greenhouse-Geisser corrected.}}\end{flushleft}
    \vspace{-8pt}
    
\end{table}
\renewcommand{\arraystretch}{1}
  



\subsubsection{Distance-based Model Factor Analysis}
\label{sec-distance_analysis}

    Using persistence threshold on distribution size, $T_{di}^S$, we calculated the \textit{differential} ($\Dspace_{di}^S$) and performed 3-factor RM ANOVA  to observe the main effects of the individual factors distribution size ($S$), number of points ($N$), and point size ($P$), as well as interaction effects (see  \autoref{tbl:factors_distance}).
        
        
    The analysis identified a significant effect of distribution size~($S$) and the number of points ($N$) on the \textit{differential} ($\Dspace_{di}^S$), but the point size~($P$) failed to reach significance. 
    In particular, we found a large effect for distribution size ($S$) on $\Dspace_{di}^S$.
    We also observed a small-medium effect in the number of points ($N$) and a negligible effect on the point size ($P$). We did not anticipate any interaction effects, and only $S*N$ showed a small effect. 
    In terms of accuracy, as pointed out in \autoref{sec-model-accuracy}, \uline{the distance-based model improved overall accuracy over using no model} (see \autoref{fig:histogram-distance}). Investigating further, \autoref{fig:di_dplot} shows the accuracy per distribution size. Note that the accuracy was sound for all distribution sizes, except at $S=85$, which negatively impacted overall performance. We speculate that this is due to the significant blending of distributions at this extreme.
    Given the large effect in $S$ and overall improvement in accuracy, \textbf{we consider \ref{Hyp:H4} confirmed}. %
        
    
    
    
    
    
    
    
    
    
    
    
    

==> sec-experiment-results.tex <==


\subsection{Results}
\label{sec-label:result}




\newcommand{\placeImageLabelA}[1]{\put(-20,45){
  		\begin{minipage}[t][0pt][t]{0pt}
			\footnotesize
			\mbox{#1}
		\end{minipage}
		}}

\newcommand{\placeImageLabelB}[1]{\put(-26,45){
  		\begin{minipage}[t][0pt][t]{0pt}
			\footnotesize
			\mbox{#1}
		\end{minipage}
		}}
		
		
		
		
\begin{figure}[!t]
    \centering

    {\begin{minipage}[t]{0.0325\linewidth}
        \rotatebox{90}{
		    \begin{minipage}{2.35cm}
		    \centering
		    \footnotesize Frequency
		    \end{minipage}
		}
	\end{minipage}}
	\begin{minipage}[t]{0.45\linewidth}	

            \includegraphics[width=0.975\linewidth]{fig/Histogram/no_model.pdf}
    \end{minipage}
    \hfill
	\begin{minipage}[t]{0.45\linewidth}
            \includegraphics[width=0.975\linewidth]{fig/Histogram/dist.pdf}
    \end{minipage}
    \hspace{2pt}
    
    \vspace{-12pt}
    \hfill
    \subfigure[Differential ($\Dspace$) without a model\label{fig:histogram-womodel}]{\hspace{0.46\linewidth}}
    \hspace{2pt}
    \subfigure[Distance-based differential ($\Dspace_{di}^S$)\label{fig:histogram-distance}]{\hspace{0.46\linewidth}}  
    
    \subfigure[Density-based differential: number of points ($\Dspace_{de}^N$), point size ($\Dspace_{de}^P$), and interaction ($\Dspace_{de}^{N*P}$)\label{fig:histogram-density}]{
    \begin{minipage}[m]{0.98\linewidth}
        \includegraphics[width=0.32\linewidth]{fig/Histogram/densN.pdf}
        \placeImageLabelA{$\Dspace_{de}^N$}
        \hfill
        \includegraphics[width=0.32\linewidth]{fig/Histogram/densP.pdf} 
        \placeImageLabelA{$\Dspace_{de}^P$}
        \hfill
        \includegraphics[width=0.32\linewidth]{fig/Histogram/densNP.pdf}
        \placeImageLabelB{$\Dspace_{de}^{N*P}$}
    \end{minipage}
    }


    \caption{Histograms for user response {differential} (horizontally) against frequency (vertically) for (a) no model (skewed due to users' underestimation), (b) the distance-based model, and (c) density-based models. Responses that are closer to $0$ imply a good fit for the data.}
    \label{fig:histogram-models}

\end{figure}







\subsubsection{Model Accuracy}
\label{sec-model-accuracy}

The distance- and density-based models both successfully estimated user perception for counting clusters. \autoref{fig:histogram-models} shows the performance of all models in terms of differential.
From our analysis, \uline{we observed the highest estimation accuracy
was achieved using the density-model}, from best to worst, $\Dspace_{de}^{N*P}$:~($\mu=0.18$, $\sigma=1.58$);  $\Dspace_{de}^{P}$:~($\mu=0.50$, $\sigma=1.67$); and $\Dspace_{de}^{N}$:~($\mu=-0.53$, $\sigma=2.14$). The distance-based model performs next best, $\Dspace_{di}^S$: ($\mu= 1.12$, $\sigma=2.64$). Whereas, without a model performed the worst, $\Dspace$: ($\mu=-3.74$, $\sigma=3.00$). 


\subsubsection{Factor Effect Analysis Without a Model}
\label{sec-visualfactorsanalysis}

We performed 3-factor RM ANOVA testing to analyze the factors, distribution size ($S$), number of points ($N$), and point size ($P$) in terms of the effect on the differential without a model, $\Dspace$. 

We observed that the \textit{distribution size}~($S$) and the \textit{number of points}~($N$) had a significant effect for counting clusters with respect to the differential, $\Dspace$, with ($F_S(4,2304)=286.11, p< 0.001, \eta^2=0.32$) and (\textcolor{green}{$F_N(1.98,1576.43)=33.98, p<0.001$}, $\eta^2=0.029$), respectively. On the other hand, \textit{data point size} ($P$) failed to reach significance, with ($F_P(3,2304)=0.21, p = 0.889$, $\eta^2=0.0002$). We also tested for interaction effects and only observed a significant effect between $S$ and $N$, ($F_{S*N}(8,2304)=8.18, p<0.001, \eta^2=0.028$).

\begin{comment}
{We observed that the \textit{distribution size}~($S$) and the \textit{number of points}~($N$) had a significant effect for counting clusters with respect to the differential, $\Dspace$, with ($F_S(4,2302)=293.88, p< 0.001, \eta^2=0.34$) and (\textcolor{green}{$F_N(1.98,1576.43)=32.98, p<0.001$}, $\eta^2=0.028$), respectively. On the other hand, \textit{data point size} ($P$) failed to reach significance, with ($F_P(3,2302)=0.32, p = 0.809$, $\eta^2=0.0004$). We also tested for interaction effects and only observed a significant effect between $S$ and $N$, ($F_{S*N}(8,2302)=8.27, p<0.001, \eta^2=0.27$). }
\end{comment}

The $\eta^2$ analysis showed a large effect size on distribution size ($S$) and a small on the number of points ($N$) and interaction effect $S*N$. This is likely because smaller distributions create denser clusters with better separation, while larger distributions blend to create ambiguous boundaries. From these results, \textbf{both \ref{Hyp:H1} and \ref{Hyp:H2} are reconfirmed}.
The lack of significance on point size ($P$) indicates that \ref{Hyp:H3} should be rejected. However, we will revisit this hypothesis later.



    
    
\input{sec-experiment-results-distance}    
\input{sec-experiment-results-density}


